Online Bayesian Persuasion Without a Clue

We study online Bayesian persuasion problems in which an informed sender repeatedly faces a receiver with the goal of influencing their behavior through the provision of payoff-relevant information. Previous works assume that the sender has knowledge about either the prior distribution over states of nature or receiver's utilities, or both. We relax such unrealistic assumptions by considering settings in which the sender does not know anything about the prior and the receiver. We design an algorithm that achieves sublinear regret with respect to an optimal signaling scheme, and we also provide a collection of lower bounds showing that the guarantees of such an algorithm are tight. Our algorithm works by searching a suitable space of signaling schemes in order to learn receiver's best responses. To do this, we leverage a non-standard representation of signaling schemes that allows to cleverly overcome the challenge of not knowing anything about the prior over states of nature and receiver's utilities. Finally, our results also allow to derive lower/upper bounds on the sample complexity of learning signaling schemes in a related Bayesian persuasion PAC-learning problem.

==> hardness.tex <==
\section{Hardness Result}
In this section we complement the study by ...  on the sample complexity of computing an approximately optimal contract. Specifically, they show that there exists an instance with $m$ outcomes and $ n = \mathcal{O} (( 1 / \epsilon) ^m) $ actions and they prove that the minimum number of samples required to learn an approximately optimal contract is of at least $\Omega ( ( 1/ \epsilon ) ^{m+2} )$. In the following we complement their study by showing that, even if the number of actions is a fixed parameter, e.g., $n=2$, the sample complexity of the computing an approximately optimal contract still depends on the the number of outcomes $m$. Specifically we show that, learning an (approximately) optimal contract requires at least $\Omega(m)$ samples as formally stated in the following.
\begin{restatable}{theorem}{hardness}
For any algorithm and for each $\epsilon > 0$, learning an $\epsilon$-optimal contracts requires at least $\Omega (m)$ samples, even with $n=2$ actions.
\end{restatable}
Theorm rules out the possibility of design an algorithm whose sample comlexity is independent from the nmber of outcomes. 

==> regret_old.tex <==
\section{The regret minimization problem}

\subsection{A no-regret algorithm}
%
Algorithm~\ref{alg:main_algorithm} is divided into three phases. In Phase~1, Algorithm~\ref{alg:main_algorithm} employs the $\texttt{Find-Search-Space}$ procedure (Algorithm~\ref{alg:estimate_prior}) to compute a subset of states of nature $\Theta' \subseteq \Theta$ in a way that it is possible to associate each signaling scheme $x \in\Delta_{d'}$ with its corresponding best response $b_x \in \A$ in few rounds, with high probability.
 
In Phase~2, Algorithm~\ref{alg:main_algorithm} employs the $ \texttt{Find-Partition}$ procedure (Algorithm~\ref{alg:find_partition}) to partition $\Delta_{d'}$ in receiver's best response regions $\preg'(a_i)$.  To do so, \dots

In Phase~3, Algorithm~\ref{alg:main_algorithm} employs the \texttt{Find-Signaling} procedure. 
%(Algorithm~\ref{alg:find_signaling_scheme}). Algorithm~\ref{alg:find_signaling_scheme} takes as input an estimate of the prior distribution and the set of separating hyperplanes computed by Algorithm~\ref{alg:find_partition}, and returns an approximately optimal signaling scheme by means of such information. Furthermore, at each round, Algorithm~\ref{alg:main_algorithm} refines the estimate of the prior by.... In this way, the signaling schemes returned by Algorithm~\ref{alg:find_signaling_scheme} become progressively closer to the optimal one.
 
Algorithm~\ref{alg:main_algorithm} guarantees the following regret bound:

\begin{restatable}{theorem}{NoRegretThm}\label{thm:no_regret_algo}
Algorithm~\ref{alg:main_algorithm} suffers regret $\mathcal{O}(d^n \sqrt T )$.
\end{restatable}


%\begin{wrapfigure}[9]{R}{0.53\textwidth}
%\vspace{-1.5cm}
%\begin{minipage}{0.53\textwidth}
\begin{algorithm}[H]
			\caption{\texttt{Main-Algorithm}}\label{alg:main_algorithm}
			\begin{algorithmic}[1]
				\Require $T \ge 0$
				\State Set $\epsilon \gets \dots $,  $p \gets \left\lceil \frac{32}{ \epsilon}\log\left(\frac{2d}{\delta} \right) \right\rceil$, $\delta \gets \dots $, $\zeta \gets \dots$
				% and $I_\theta \gets 0 \,\, \forall \theta \in \Theta$
				\State $\left( \hat \mu, \Theta' \right) \gets \texttt{Find-Search-Space}(p)$ %\Comment{\textcolor{gray}{Phase 1}}
				\State Set $d' \gets |\Theta'|$			
				\State $ \mathcal{V} \gets \texttt{Find-Partition}(\Delta_{d'}, \zeta)$ %\Comment{\textcolor{gray}{Phase 2}}
				\While{$\tau \le T$} %\Comment{\textcolor{gray}{Phase 3}}
				\State $\phi^\tau \gets \texttt{Find-Signaling} (\mathcal{V},\Theta', \hat \mu ) $  %\Comment{\textcolor{gray}{Phase 3}}
				\State The sender commits to $\phi^{\tau}$, samples $\theta \sim \mu$ and set $N_\theta \gets N_\theta  +1$ 
				\State Set $\hat \mu_{\theta} = N_{\theta} / \sum_{\theta \in \Theta'} N_{\theta}$ for each $\theta \in \Theta' $
				%\State Set $\hat{\mu}_{\theta} \gets N_{\theta} /\ \sum_{\theta \in \theta} N_{\theta} \,\,\ \forall \theta \in \Theta$ 
				\EndWhile
			\end{algorithmic}
		\end{algorithm}
%\end{minipage}
%\end{wrapfigure}
%
%\subsubsection{Phase 1:  \texttt{Find-Search-Space}}
%%
%The main goal of the \texttt{Find-Search-Space} procedure (Algorithm~\ref{alg:estimate_prior}) is to compute a suitable set of states of nature $\Theta \subseteq \Theta'$, in a way to associate each signaling scheme $x \in \Delta_{d'}$ with its corresponding best response $b_x \in \mathcal{A}$ in at most $\mathcal{O}(\nicefrac{1}{\epsilon})$ rounds, with high probability. To do so, Algorithm~\ref{alg:estimate_prior} employs $p \in \mathbb{N}_{+}$ rounds at Lines~\ref{line:compute_prior_begin}-\ref{line:compute_prior_end} to compute an estimate of the prior distribution.
%%	\begin{wrapfigure}[13]{R}{0.53\textwidth}
%%	\vspace{-1.3cm}
%%	\begin{minipage}{0.53\textwidth}
%		\begin{algorithm}[H]
%			\caption{\texttt{Find-Search-Space}}\label{alg:estimate_prior}
%			\begin{algorithmic}[1]
%				\Require $p \in \mathbb{N}_{+}$
%				\State Set $\Theta ' \gets \{\emptyset\}$ and $N_\theta \gets 0 \,\, \forall \theta \in \Theta$
%				\For{$\tau = 1 \dots p$} \label{line:compute_prior_begin}
%				\State Commit to any signaling scheme $\phi^{\tau}$
%				\State Sample $\theta \sim \mu$ and set $N_\theta \gets N_\theta  +1$
%				\EndFor
%				\State $\hat{\mu}_{\theta} \gets {N_{\theta}}/ {p} \,\,\ \forall \theta \in \Theta$ \label{line:compute_prior_end}
%				\For{$\theta \in \Theta$}
%				\State  \textbf{if} $\hat{\mu}_{\theta} >  2\epsilon$ \textbf{then} $\Theta'\gets \Theta' \cup \{ \theta \}$\label{line:set_Theta} 	
%				\EndFor  
%				 %\mathcal{X}_\epsilon \gets \Delta_{d'} \cap \left\{ x \in \mathbb{R}_+^{d'} \mid \sum_{\theta  \in \Theta'} \hat{\mu}_{\theta}x_\theta \ge 2\epsilon \right\}$\label{line:set_xi_defintion}
%				\State \textbf{return} $\left( \hat \mu, \Theta' \right)$						
%			\end{algorithmic}
%		\end{algorithm}
%%	\end{minipage}
%%\end{wrapfigure}
%%
%Thanks to the multiplicative version of the Chernoff bound we can distinguish in $\mathcal{O}(\nicefrac{1}{\epsilon})$ rounds if the components of the prior distribution are smaller than the given threshold $\epsilon$. Such a technical component is necessary to avoid using $\mathcal{O}(\nicefrac{1}{\epsilon^2})$ rounds to estimate the prior by employing standard concentration inequalities. Thus, at Lines~\ref{line:set_Theta}, Algorithm~\ref{alg:estimate_prior} computes a set of states of nature $\Theta' \subseteq \Theta$, ensuring that if $\theta \in \Theta'$, then the probability of sampling such a state is greater than $\epsilon > 0$, and the empirical mean of each $\hat{\mu}_\theta$ with $\theta \in \Theta'$ is guaranteed to belong to a suitable confidence interval, with high probability.
%%
%Formally:
%%
%\begin{restatable}{lemma}{PriorEstimate}\label{lem:prior_estimate} 
%	With probability at least $1-\delta$ in $p = \left\lceil \nicefrac{12}{ \epsilon}\log\left(\nicefrac{2d}{\delta} \right) \right\rceil$ rounds, Algorithm~\ref{alg:estimate_prior} computes a set $\Theta' \subseteq \Theta$ such that if $\mu_{\theta} \le \epsilon$, then $\theta \not \in \Theta'$, while if $\mu_{\theta} \ge 4\epsilon$ then $\theta \in \Theta'$. %Furthermore, for each $\theta \in \Theta'$, it holds $\hat{\mu}_\theta/2  \le \mu_\theta \le 3\hat{\mu}_\theta/2$. % Furthermore, for each $\theta \in \Theta' $ we have that $\mu_{\theta}/2 \le\hat\mu_{\theta} \le 2\mu_{\theta}$. 
%\end{restatable}
%%
%We also introduce the definition of the \emph{clean event} of Phase~1, as formally stated below.
%%
%\begin{definition}[Clean event of Phase~1]
%	We let $\mathcal{E}^1$ be the event under which all the elements $\theta \in \Theta'$ are such that $\hat{\mu}_\theta/2  \le \mu_\theta \le 3\hat{\mu}_\theta/2$. Furthermore, if $\theta \in \Theta' $, then $\mu_\theta \ge \epsilon$, while if  $\theta \not \in \Theta' $, then $\mu_\theta \le 4\epsilon$.
%\end{definition}
%%
%Intuitively, under the clean event $\mathcal{E}^1$, all the components of $\hat{\mu}$ have been estimated well, and, thus, the set $\Theta' \subseteq \Theta$ contains only those states occurring with a probability greater than $\epsilon>0$. As a result, under the event $\mathcal{E}^1$, the following lemma holds.
%%
%\begin{restatable}{lemma}{PriorRounds}\label{lem:rounds_signal} 
%	Under the event  $\mathcal{E}^1$, given $\rho > 0$ and any two signals signaling scheme $x \in \Delta_{d'}$, if the sender commits to the same signaling scheme $x$ for at least $q \coloneqq \left\lceil \nicefrac{\log(\rho)}{\log(1-\epsilon)} \right \rceil$ rounds, then the probability of observing the signal $s_1$ is at least $1-\rho$.
%\end{restatable}
\subsubsection{Phase 1:  \texttt{Find-Search-Space}}
%
The main goal of the \texttt{Find-Search-Space} procedure (Algorithm~\ref{alg:estimate_prior}) is to compute a suitable set of two signaling schemes $\mathcal{X}_\epsilon$, in a way that each signaling scheme $x \in \mathcal{X}_\epsilon$, observes the best response $b_x \in \mathcal{A}$ in at most $\mathcal{O}(\nicefrac{1}{\epsilon})$ rounds, with high probability. To do so, Algorithm~\ref{alg:estimate_prior} at Lines~\ref{line:compute_prior_begin}-\ref{line:compute_prior_end} employs $p\in \mathbb{N}_{+}$ rounds to compute an estimate of the prior distribution.
%	\begin{wrapfigure}[13]{R}{0.53\textwidth}
	%	\vspace{-1.3cm}
	%	\begin{minipage}{0.53\textwidth}
		\begin{algorithm}[H]
			\caption{\texttt{Find-Search-Space}}\label{alg:estimate_prior}
			\begin{algorithmic}[1]
				\Require $p \in \mathbb{N}_{+}$
				\State Set $\Theta ' \gets \{\emptyset\}$ and $N_\theta \gets 0 \,\, \forall \theta \in \Theta$
				\For{$\tau = 1 \dots p$} \label{line:compute_prior_begin}
				\State Commit to any signaling scheme $\phi^{\tau}$
				\State Sample $\theta \sim \mu$ and set $N_\theta \gets N_\theta  +1$
				\EndFor
				\State $\hat{\mu}_{\theta} \gets {N_{\theta}}/ {p} \,\,\ \forall \theta \in \Theta$ \label{line:compute_prior_end}
				\For{$\theta \in \Theta$}
				\State  \textbf{if} $\hat{\mu}_{\theta} >  2\epsilon$ \textbf{then} $\Theta'\gets \Theta' \cup \{ \theta \}$\label{line:set_Theta} 	
				\EndFor  
				\State Set $d' \gets |\Theta'|$
				%\mathcal{X}_\epsilon \gets \Delta_{d'} \cap \left\{ x \in \mathbb{R}_+^{d'} \mid \sum_{\theta  \in \Theta'} \hat{\mu}_{\theta}x_\theta \ge 2\epsilon \right\}$\label{line:set_xi_defintion}
				\State \textbf{return} $\left( \hat \mu, \mathcal{X}_\epsilon, \Theta' \right)$						
			\end{algorithmic}
		\end{algorithm}
		%	\end{minipage}
	%\end{wrapfigure}
	%
	%We observe that a standard approach to compute an estimate of the different components of the prior distribution would require employing the well-known Hoeffding inequality so that the final estimates are within $\epsilon$ close to the original ones with high probability. However, this would require to employ $\mathcal{O}({1}/{\epsilon^2})$ rounds, thus preventing our algorithm to achieve the desired regret guarantees.
	Thanks to the multiplicative version of the Chernoff bound we can distinguish in $\mathcal{O}({1}/{\epsilon})$ rounds if the components of the prior distribution are smaller than the given threshold $\epsilon$. Such a technical component is necessary to avoid using $\mathcal{O}(\nicefrac{1}{\epsilon^2})$ rounds to estimate the prior by employing standard concentration inequalities. Thus, at Lines~\ref{line:set_Theta}, Algorithm~\ref{alg:estimate_prior} computes a set of states of nature $\Theta' \subseteq \Theta$ ensuring that if $\theta \in \Theta'$, then the probability of sampling such a state is greater than $\epsilon$ with high probability, and the empirical mean of each  $\hat{\mu}_\theta$ with  $\theta \in \Theta'$ is guaranteed to belong to a suitable confidence interval. Formally:
	%
	\begin{restatable}{lemma}{PriorEstimate}\label{lem:prior_estimate} 
		With probability at least $1-\delta$ in $p = \left\lceil \nicefrac{12}{ \epsilon}\log\left(\nicefrac{2d}{\delta} \right) \right\rceil$ rounds, Algorithm~\ref{alg:estimate_prior} computes a set $\Theta' \subseteq \Theta$ such that if $\mu_{\theta} \le \epsilon$, then $\theta \not \in \Theta'$, while if $\mu_{\theta} \ge 4\epsilon$ then $\theta \in \Theta'$. Furthermore, for each $\theta \in \Theta'$, it holds $\hat{\mu}_\theta/2  \le \mu_\theta \le 3\hat{\mu}_\theta/2$. % Furthermore, for each $\theta \in \Theta' $ we have that $\mu_{\theta}/2 \le\hat\mu_{\theta} \le 2\mu_{\theta}$. 
	\end{restatable}
	%
	We also introduce the definition of the \emph{clean event} of Phase~1, as formally stated below.
	%
	\begin{definition}[Clean event of Phase~1]
		We let $\mathcal{E}^1$ be the event under which all the elements $\theta \in \Theta'$ are such that $\hat{\mu}_\theta/2  \le \mu_\theta \le 3\hat{\mu}_\theta/2$. Furthermore, if $\theta \in \Theta' $, then $\mu_\theta \ge \epsilon$, while if  $\theta \not \in \Theta' $, then $\mu_\theta \le 4\epsilon$.
	\end{definition}
	%
	Intuitively, under the clean event $\mathcal{E}^1$, all the components of $\hat{\mu}$ have been estimated well, and, thus, the set $\Theta'$ contains only those states occurring with a probability greater than $\epsilon$. Thus, under the event $\mathcal{E}^1$, Algorithm~\ref{alg:estimate_prior} computes at Line~\ref{line:set_xi_defintion} a set $\mathcal{X}_\epsilon \subseteq \mathcal{C}_{d'} \cap \Delta_{d'}$ such that each element $x \in \mathcal{X}_\epsilon$ samples in a number of rounds, which is of the order $\mathcal{O}({1}/{\epsilon})$, the signal $s_1 \sim x_\theta$ for at least one $\theta \in \Theta'$ with high probability. In such a way, in at most $\mathcal{O}(1/\epsilon)$ rounds, it is possible to associate to each $x \in \mathcal{X}_\epsilon$ its corresponding best response $b_x \in \mathcal{A}$, with high probability. Formally, the following lemma holds.
	%
	\begin{restatable}{lemma}{PriorRounds}\label{lem:rounds_signal} 
		Under the event  $\mathcal{E}^1$, given $\rho > 0$ and any two signals signaling scheme $x \in \mathcal{X}_\epsilon$, if the sender commits to the same signaling scheme $x$ for at least $q \coloneqq \left\lceil \nicefrac{\log(\rho)}{\log(1-\epsilon)} \right \rceil$ rounds, then the probability of observing the signal $s_1$ is at least $1-\rho$.
	\end{restatable}

\begin{comment}
		%Given $\delta >0$, then in at most $q \coloneqq \left\lceil \frac{\log(\delta)}{\log(1-\epsilon)} \right \rceil $ rounds, Algorithm~\ref{alg:action_oracle} returns the action $b_{\xi^{s_1}} \in \mathcal{A}$, with probability of at least $1-\delta$.
	%and $O\left(\nicefrac{\log(d/\delta)}{\epsilon}\right)$ rounds, Algorithm~\ref{alg:estimate_prior} computes a set $\Theta' \subseteq \Theta$ such that for each $\theta \in \Theta $ with $\mu_{\theta} \le \epsilon$, then $\theta' \not \in \Theta'$. Furthermore, for each $\theta \in \Theta $ such that $\mu_{\theta} \ge 4\epsilon$, then $\theta \in \Theta'$. 
\subsection{\texttt{Action-Oracle}}\label{sec:action_oracle}

Given a posterior $\xi \in \Delta_{\Theta}$ as input, the goal of the  \texttt{Action-Oracle} procedure is to determine the best response associated to it. In contrast to Stackelberg games, the sender cannot directly commit to $\xi \in \Xi$, as they can only commit to a signaling scheme $\gamma$ that includes it in its support. Consequently, we propose a procedure that allows us to associate to each posterior distribution $\xi \in \Xi$ its corresponding best response with high probability.

In the initial phase of Algorithm~\ref{alg:action_oracle} (Lines~\ref{line:action_or_first}--\ref{line:action_or_first_last}), we construct a signaling scheme $\gamma$ in a way that the posterior distribution $\xi^1$ given as input to \texttt{Action-Oracle} belongs to the support of $\gamma$, \emph{i.e.}, $\gamma(\xi^1)>0$. Clearly, our aim is to design a signaling scheme where $\gamma(\xi^1)$ is as large as possible. However, the consistency constraints (See Equation~3), limit the possibility of assigning arbitrarily large values to $\gamma(\xi^*)$.  As a consequence, we set $\gamma(\xi^1)$ equal to the ratio between $\mu_{\theta^1  } $ and $ \xi^1_{\theta^1}$ where $\theta^* \in \theta$ is the state of nature ensuring that $\gamma(\xi^*){\xi}^*_{\theta}$ is less or equal to $\mu_\theta$ for each $\theta \in \Theta$. Then, we let be the support of $\gamma$ be defined by all the posteriors with unitary probability in a state $\theta$ for all $\theta \in \Theta \setminus \{\theta^*\}$. In the following, we show that the signaling scheme defined by \texttt{Action-Oracle} in Equation~\ref{eq:signaling_scheme} is actually a signaling scheme, \emph{i.e.}, and it is a consistent distribution over its support and satisfies Equations. 
\begin{restatable}{lemma}{boundedactions}\label{lem:boundedactions}
	In Algorithm \dots, Equation~\ref{eq:signaling_scheme} defines a signaling scheme $\gamma \in \Delta_{\Xi}$ satisfying Equation 
\end{restatable}
\begin{proof}
\begin{enumerate}
\item $\sum_{\xi \in \textnormal{supp}(\gamma)} \gamma_\xi   = 1$
\begin{align*}
	\sum_{\xi \in \textnormal{supp}(\gamma)} \gamma(\xi ) &= 	  \sum_{\theta \in \widetilde{\Theta}} \gamma_{\mathbb{I}(\theta)} + \gamma_{\xi^*} \\
	 &= \sum_{\theta \in \widetilde{\Theta}} \left( \mu_{\theta} - \gamma_{\xi^*} {{\xi}_{\theta}^*} \right)  + \gamma_{\xi^*}  \\	
	&= \sum_{\theta \in \widetilde{\Theta}} \mu_{\theta}  + \gamma_{\xi^*}  \left( 1- \sum_{\theta \in \widetilde{\Theta}} \xi_\theta^*
	\right) \\	
	&= \sum_{\theta \in \widetilde{\Theta}} \mu_{\theta}  + \gamma_{\xi^*} \xi_{\theta^*}^*  = \sum_{\theta \in \widetilde{\Theta}} \mu_{\theta}  + \mu_{\theta^*} = 1  \\	
\end{align*}
\item $\sum_{\xi \in \textnormal{supp}(\gamma)} \gamma_\xi  \xi _\theta  = \mu_\theta \,\,\,\ \forall \theta \in \Theta$
\begin{align*}
	\sum_{\xi \in \textnormal{supp}(\gamma)} \gamma_\xi  \xi _{\theta^*}  &= \gamma_{\xi^*}   \xi^* _{\theta^*} =  \mu_{\theta^*} \\	
	\sum_{\xi \in \textnormal{supp}(\gamma)} \gamma_\xi  \xi _\theta & = \gamma_{\mathbb{I}(\theta)}   \mathbb{I}(\theta) + \gamma(\xi^*)  \xi^* _{\theta} =  \mu_\theta - \gamma_\xi^* \xi_{\theta}^*  + \gamma_\xi^* \xi_{\theta}^*  = \mu_\theta \,\,\, \forall \theta \in \widetilde{\Theta}\\	
\end{align*}

\item $\gamma(\xi ) \ge 0  \,\,\,\ \forall  \xi \in \textnormal{supp}(\gamma) $. We notice that $\gamma(\xi^* ) \ge 0$ by definition. While, for all $\theta \in \widetilde{\Theta}$ we have:
\begin{equation*}
	\gamma_{\mathbb{I}(\theta)}   = 	\mu_\theta -   \frac{\mu_{\theta^*}}{{\xi}_{\theta^*}^*}  {\xi}_{\theta}^* \ge  \mu_\theta -   \frac{\mu_{\theta}}{{\xi}_{\theta}^*}  {\xi}_{\theta}^* = 0
\end{equation*}

\end{enumerate}
\end{proof}

In the second phase of Algorithm~\ref{alg:action_oracle} we commit to signaling scheme $\gamma$ computed and at each round we sample $\xi $ from $\gamma$. Such a smpling procedure terinate when either the posterior drawn from $\gamma$ coincides with $\xi_1$. Lemma provides the number of rounds to compte an approximately optimal sgnaling scheme with high probability.  




	\begin{algorithm}[H]
	\caption{\texttt{Action-Oracle}}\label{alg:action_oracle}
	\begin{algorithmic}[1]
		\Require posterior $\xi^* \in \Xi$
		\State Define $\gamma \in \Delta_\Xi$ as follows:
		\State Define $\theta^* \in \argmin_{\theta \in \Theta} \frac{\mu_{\theta}}{{\xi}_{\theta}^*} $ and $\widetilde{\Theta} \coloneqq \Theta \setminus \{ \theta^* \}$
	\State Define $\textnormal{supp}(\gamma) \coloneqq \{ \xi^* \} \cup  \{ \mathbb{I}(\theta)   \}_{\theta \in \widetilde{\Theta} }$
		
	\end{algorithmic}
\end{algorithm}

\begin{comment}
	
	
	
%n the first phase (Lines~\ref{line:action_or_first}--\ref{line:action_or_first_last}), Algorithm~\ref{alg:action_oracle} prescribes the principal to commit to the contract $p \in \preg$ given as input for $q \in \mathbb{N}$ consecutive rounds (see the proof of Theorem~\ref{thm:finalthm} for the definition of $q$).
%
This is done to build an empirical distribution $\widetilde{F} \in \Delta_{\Omega}$ that estimates the (true) distribution over outcomes $F_{a^\star(p)}$ induced by the agent's best response $a^\star(p)$.
%
In the second phase (Lines~\ref{line:action_or_second}--\ref{line:action_or_second_last}), such an empirical distribution is compared with those computed during previous calls to Algorithm~\ref{alg:action_oracle}, in order to decide whether $a^\star(p)$ can be safely mapped to some $d \in \mathcal{D}$ or \emph{not}.
%
To perform such a comparison, all the empirical distributions computed by the algorithm are stored in a dictionary $\mathcal{F}$ (initialized in Line~\ref{line:set_D_F} of Algorithm~\ref{alg:final_algorithm}), where $\mathcal{F}[d]$ contains all the $\widetilde{F} \in \Delta_{\Omega}$ associated with $d \in \mathcal{D}$.
%
%computed by Algorithm~\ref{alg:action_oracle} when it concluded that the agent's best response can be safely associated with $d \in \mathcal{D}$.
%
% all the $\widetilde{F} \in \Delta_{\Omega}$ computed by Algorithm~\ref{alg:action_oracle} for contracts $p \in \mathcal{P}$ whose corresponding best response $a^\star(p)$ is associated with $d \in \mathcal{D}$.



The first phase of Algorithm~\ref{alg:action_oracle} ensures that $ \|  \widetilde F - F_{a^\star(p)} \|_{\infty} \le \epsilon $ holds with sufficiently high probability.
%
For ease of presentation, in the following definition we introduce a \emph{clean event} that allows us to factor out from our analysis the ``with high probability'' statements.
%
In Section~\ref{sec:final_algo}, we will show that such an event holds with sufficiently high probability given how the value of $q$ is chosen.
%
\begin{definition}[Clean event]
	Given any $\epsilon > 0$, we let $\mathcal{E}_\epsilon$ be the event in which Algorithm~\ref{alg:action_oracle} always computes some $\widetilde F \in \Delta_{\Omega}$ such that $ \|\widetilde{F} - F_{a^\star(p)} \|_{\infty} \le \epsilon $, where $p \in \mathcal{P}$ is the input to the algorithm.
\end{definition}



%
In the second phase, Algorithm~\ref{alg:action_oracle} searches for all the meta-actions $d \in \mathcal{D}$ such that $\mathcal{F}[d]$ contains \emph{at least one} empirical distribution which is ``sufficiently close'' to the $\widetilde{F}$ that has just been computed by the algorithm.
%
%associated with \emph{at least one} (previously-computed) empirical distribution that is ``sufficiently close'' to $\widetilde{F}$.
%
Formally, the algorithm looks for all the meta-actions $d \in \mathcal{D}$ such that $ \| F -   \widetilde F \|_{\infty} \le 2 \epsilon $ for at least one $F \in \mathcal{F}[d]$.
%
Then, three cases are possible:
%
\begin{itemize}[leftmargin=6mm]
	\item If the algorithm finds a \emph{unique} $d \in \mathcal{D}$ with such a property (case $|\mathcal{D}^\diamond|=1$), then $d$ is returned since $a^\star(p)$ can be safely mapped to $d$.
	%
	\item If the algorithm does \emph{not} find any meta-action $d \in \mathcal{D}$ with such a property (case $\mathcal{D}^\diamond=\varnothing$), then a new meta-action $d^\diamond$ is added to $\mathcal{D}$.
	% so that $a^\star(p)$ can be safely associated with it.
	%
	\item If the algorithm finds \emph{more than one} meta-action $d \in \mathcal{D}$ with such a property ($|\mathcal{D}^\diamond| > 1$), then all the meta-actions in $\mathcal{D}^\diamond$ are merged into a single (new) meta-action $d^\diamond$.
	% so that $a^\star(p)$ can be safely associated with it.
\end{itemize}
%
%
In Algorithm~\ref{alg:action_oracle}, the last two cases above are jointly managed by Lines~\ref{line:new_meta}--\ref{line:action_or_second_last}, and in both cases the algorithm returns the special value $\bot$.
%
This alerts the calling procedure that the set $\mathcal{D}$ has changed, and, thus, the \texttt{Try-Cover} procedure needs to be re-started.
%
Notice that Algorithm~\ref{alg:action_oracle} also takes care of properly updating the dictionary $\mathcal{F}$, which is done in Lines~\ref{line:add}~and~\ref{line:clear}.
%
Moreover, whenever Algorithm~\ref{alg:action_oracle} adds a new meta-action $d^\diamond$ into $\mathcal{D}$, this is also associated with a particular empirical distribution $\widetilde{F}_{d^\diamond}$, which is set to be equal to $\widetilde{F}$ (Line~\ref{line:assoc_ditrib}).
%
% for ease of exposition, whenever Algorithm~\ref{alg:action_oracle} adds a new meta-action $d$ into $\mathcal{D}$, this is associated with an empirical distribution $\widetilde{F}_{d}$ equal to the $\widetilde{F}$ that has just been computed (Line~\ref{line:assoc_ditrib}).
%
We remark that the symbols $\widetilde{F}_d$ for $d \in \mathcal{D}$ have only been introduced for ease of exposition, and they do \emph{not} reference actual variables declared in the algorithm.
%
Operationally, one can replace each appearance of $\widetilde{F}_d$ in the algorithms with any fixed empirical distribution contained in the dictionary entry $\mathcal{F}[d]$.
%
% $\widetilde{F}_d$ does \emph{not} correspond to any variable.
%
% Operationally, one can use any element in $\mathcal{F}[d]$ instead.
%
% This will be needed by the \texttt{Try-Partition} and the \texttt{Find-Contract} procedures.\footnote{Let us remark that the symbols $\widetilde{F}_d$ for $d \in \mathcal{D}$ have been introduced for ease of exposition, and, thus, they do \emph{not} correspond to actual variables. Indeed, one may use any empirical distribution in $\mathcal{F}[d]$ in place of $\widetilde{F}_d$.}


The first crucial property that Algorithm~\ref{alg:action_oracle} guarantees is that \emph{only ``similar'' agent's best-response actions are mapped to the same meta-action}.
%
In order to formally state such a property, we first need to introduce the definition of set of agent's actions \emph{associated with} a meta-action in $\mathcal{D}$.
%
%
% the algorithm returns a meta-action $d \in \mathcal{D}$, then the agent's best response $a^\star(p)$ in the contract $p \in \mathcal{P}$ given as input can be safely associated with $d$.
%
% , whenever the agent's best response $a^\star(p)$ can be safely associated with some meta-action in $\mathcal{D}$, then the algorithm correctly returns such a meta-action.
%
% In order to state such a property, we first need to formally introduce the set of agent's actions \emph{associated with} a meta-action in $\mathcal{D}$, which is defined as follows: 
%
% Formally, the set of agent's actions \emph{associated with} a meta-action in $\mathcal{D}$ is defined as follows: 
%
%\begin{definition}[Associated actions]\label{def:associated_actions}
%	For every $d \in \mathcal{D}$, let $\mathcal{P}_d \subseteq \mathcal{P}$ be the set of contracts $p \in \mathcal{P}$ that are given as input to Algorithm~\ref{alg:action_oracle} in all the calls in which it computed an empirical distribution $\widetilde F \in \mathcal{F}[d]$.
%	%
%	Then, we define the set of actions \emph{associated with} a meta-action $d \in \mathcal{D}$ as $I(d) \coloneqq \bigcup_{p \in \mathcal{P}_d} a^\star(p)$ .
%\end{definition}
%
\begin{definition}[Associated actions]\label{def:asssoc_actions}
	Given a set $\mathcal{D}$ of meta-actions and a dictionary $\mathcal{F}$ of empirical distributions computed by means of Algorithm~\ref{alg:action_oracle}, we let $A: \mathcal{D} \to 2^\mathcal{A}$ be a function such that $A(d)$ represents the \emph{set of actions associated with} the meta-action $d \in \mathcal{D}$, defined as follows:
	\[
	A(d) = \left\{a \in \mathcal{A} \mid  \,\, \rVert \widetilde{F}_d -  F_a  \lVert_\infty\le 5 \epsilon n \wedge \exists p \in \mathcal P: a=a^\star(p) \right\}.
	\]
	%	
	%	Given a distribution $F \in \Delta_\Omega$, we let $B(F)\subseteq \mathcal{A}$ be set
	%	\[\{a \in A: \rVert F_a-F\lVert_\infty\le 5 \epsilon n \wedge \exists p \in \mathcal P: a=a^*(p)\}\]
\end{definition}
%
The set $A(d)$ encompasses all the agent's actions $a \in \mathcal{A}$ whose distributions over outcomes $F_a$ are ``similar'' to the empirical distribution $\widetilde{F}_d$ associated with the meta-action $d \in \mathcal{D}$, where the entity of the similarity is defined in a suitable way depending on $\epsilon$ and the number of agent's actions $n$.
%
Moreover, notice that the set $A(d)$ only contains agent's actions that can be induced as best response for at least one contract $p \in \mathcal{P}$.
%
This is needed in order to simplify the analysis of the algorithm.
%
Let us also remark that an agent's action may be associated with \emph{more than one} meta-action.
%
% In particular, whenever the algorithm returns a meta-action $d \in \mathcal{D}$ for a contract $p \in \mathcal{P}$ given as input, then the agent's best response $a^\star(p)$ is indeed associated with the meta-action $d$.
%
Equipped with Definition~\ref{def:asssoc_actions}, the property introduced above can be formally stated as follows:
%
\begin{restatable}{lemma}{boundedactions}\label{lem:boundedactions}
	Equation~\ref{eq:signaling_scheme} define a signaling scheme $\gamma \in \Delta_{\Xi}$ satisfying Equation 
\end{restatable}
%
Intuitively, Lemma~\ref{lem:boundedactions} follows from the observation that, under the event $\mathcal{E}_\epsilon$, the empirical distributions computed by Algorithm~\ref{alg:action_oracle} are ``close'' to the true ones, and, thus, the distributions over outcomes of all the actions associated with $d$ are sufficiently ``close'' to each other.
%
A non-trivial part of the proof of Lemma~\ref{lem:boundedactions} is to show that Algorithm~\ref{alg:action_oracle} does \emph{not} put in the same dictionary entry $\mathcal{F}[d]$ empirical distributions that form a ``chain" growing arbitrarily long in terms of $\lVert \cdot \rVert_\infty$ norm, but instead the length of such ``chains" is always bounded by $5 \epsilon n$.  
%
% ensures that there are no ``chains" of empirical distributions that grow arbitrarily, but the length of such ``chains" can be bounded by the number of actions.
%
%the proof follows noticing that under the event $\mathcal{E}_\epsilon$, the empirical distributions induced by the actions are close to the real one, and all the empirical distributions in $\mathcal{F}[d]$ are close.
%The non-trivial part of the proof is to show that there do not exist "chains" of empirical distributions close only in pairs. We show that the length of these chains is bounded by the number of actions.
%
% Indeed, Algorithm~\ref{alg:action_oracle} assigns to the same meta-action only actions that are at most close to at least another action. Hence, 

% \ldots \alb{Dare intuizione proof, non capisco più un cazzo di come è la proof adesso}
%\bac{Intuitively, the lemma follows by observing that, under the event $\mathcal{E}_\epsilon$, the agent's action $a_i$ leading to the empirical distribution $\widetilde{F}_d$ is sufficiently close to $F_{a_i} $. Furthermore, by noticing that all the agent's actions implemented by a contract $p$ in which \texttt{Action-Oracle} returns the meta-action $d$ must satisfy the condition $\| F_{a^\star(p)} - F_{a_i}\|_\infty  \le 4 \epsilon n$.}


The second crucial property of Algorithm~\ref{alg:action_oracle} is made formal by the following lemma:
%
\begin{restatable}{lemma}{finaliterations}\label{lem:finaliterations}
	Under the event $\mathcal{E}_\epsilon$, Algorithm~\ref{alg:action_oracle} returns $\bot$ at most $2n$ times.
	%
	%The number of iterations required \textnormal{\texttt{Discover-and-Partition}} is of at most $2n$.
\end{restatable}
%
Intuitively, Lemma~\ref{lem:finaliterations} follows from the fact that Algorithm~\ref{alg:action_oracle} increases the cardinality of the set $\mathcal{D}$ by one only when $\|  F - \widetilde{F} \|_\infty > 2 \epsilon$ for all ${F} \in \mathcal{F}[d]$ and $d \in \mathcal{D}$.
%
In such a case, under the event $\mathcal{E}_\epsilon$ the agent's best response is an action that has never been played before.
%
Thus, the cardinality of $\mathcal{D}$ can be increased at most $n$ times.
%
Moreover, in the worst case the cardinality of $\mathcal{D}$ is reduced by one for $n$ times, resulting in $2 n $ being the maximum number of times Algorithm~\ref{alg:action_oracle} returns $\bot$.


All the actions associated with the same meta-action also enjoy a useful property concerning their costs.
%
In particular, we formally introduce the following definition of \emph{cost of a meta-action}:
%
\begin{definition}[Cost of a meta-action]\label{def:cost_action}
	Given a set $\mathcal{D}$ of meta-actions and a dictionary $\mathcal{F}$ of empirical distributions computed by means of Algorithm~\ref{alg:action_oracle}, we let $c: \mathcal{D} \to [0,1]$ be a function such that $c(d)$ represents the \emph{cost of meta-action} $d \in \mathcal{D}$, defined as $c(d) = \min_{a \in A(d)} c_{a}$.
\end{definition}
%
%\begin{definition}[close of a distribution]
%	Given a distribution $F\in \Delta_\Omega$, we let $c(d)= \min_{a \in A(d)} c_{a}$.
%\end{definition}
%
Then, we can prove the following lemma:
%
% Interestingly, given a distribution $F$, actions in $B(F)$ have cost close to $c_{F}$.
%
\begin{restatable}{lemma}{costactions}\label{lem:cost_actions}
	Given a set $\mathcal{D}$ of meta-actions and a dictionary $\mathcal{F}$ of empirical distributions computed by means of Algorithm~\ref{alg:action_oracle}, under the event $\mathcal{E}_\epsilon$, for every meta-action $d \in \mathcal{D}$ and associated action $a \in A(d)$ it holds that $|c(d) - c_a| \le 4 B \epsilon m n$.
	%
	% Under the event $\mathcal{E}_\epsilon$, given a meta-action $d \in \mathcal{D}$, for each $a \in A(d)$ it holds $|c(d) - c_a| \le 4 \epsilon n$.
\end{restatable}
%
Moreover, by Lemma~\ref{lem:cost_actions} and Holder's inequality, we can readily prove the following lemma, which will be useful in proving many of ours results. 
%
\begin{restatable}{lemma}{closeutility}\label{lem:utility_closed}
	Given a set $\mathcal{D}$ of meta-actions and a dictionary $\mathcal{F}$ of empirical distributions computed by means of Algorithm~\ref{alg:action_oracle}, under the event $\mathcal{E}_\epsilon$, for every meta-action $d \in \mathcal{D}$, associated action $a \in A(d)$, and contract $p \in \mathcal{P}$ it holds
	$
	| \sum_{\omega \in \Omega} \widetilde{F}_{d,\omega} \, p_\omega -c(d) - \sum_{\omega \in \Omega} F_{a, \omega} \, p_\omega + c_{a}  | \le 9B\epsilon m n.
	$
	%	\begin{equation*}
		%		\left| \left( \sum_{\omega \in \Omega} \widetilde{F}_{d,\omega} \, p_\omega -c(d) \right) - \left(\sum_{\omega \in \Omega} F_{a, \omega} \, p_\omega- c_{a}\right)\right| \le 9B\epsilon m n.
		%	\end{equation*}
	%	
	%	Under the event $\mathcal{E}_\epsilon$, given a meta-action $d \in \mathcal{ D}$, for each $a \in A(d)$ and $p \in \mathcal{P}$ it holds:
	%	\begin{equation*}
		%	\left|\sum_{\omega \in \Omega} \widetilde{F}_{d,\omega} p_\omega -c(d) - \left(\sum_{\omega \in \Omega} F_{a, \omega} p_\omega- c_{a}\right)\right| \le X.
		%	\end{equation*}
\end{restatable}





%Intuitively, Lemma~\ref{lem:nullintersection} holds thanks to the following observation.
%%
%If Algorithm~\ref{alg:action_oracle} is run for two contracts $p, p' \in \mathcal{P}$ such that $a^\star(p) = a^\star(p')$, then the computed empirical distributions are guaranteed to be within $2\epsilon$ of each other (in norm $\| \cdot\|_\infty$) under the clean event $\mathcal{E}_\epsilon$.
%%
%Thus, in the case $|\mathcal{D}^\diamond|=1$, the property is clearly preserved by the algorithm.
%%
%Moreover, in the other two cases, the property is preserved as well given how the set $\mathcal{D}$ is updated by the algorithm.
%
%
%The second crucial property of Algorithm~\ref{alg:action_oracle} is that only actions inducing ``similar'' distributions over outcomes can be associated with the same meta-action.
%%
%Formally:
%%Such a property is formally stated by the following lemma:
%%
%
%
%
%%
%Intuitively, Lemma~\ref{lem:boundedactions} follows from the observation that, if the distributions $F_a, F_{a'}$ of two different actions $a, a' \in \mathcal{A}$ are ``sufficiently far part'', then such actions are never associated with the same meta-action by Algorithm~\ref{alg:action_oracle}, under the event $\mathcal{E}_\epsilon$.
%%
%This holds thanks to how a new meta-action $d^\diamond$ is ``built'' by the algorithm, when either $\mathcal{D}^\diamond=\varnothing$ or $|\mathcal{D}^\diamond| > 1$.






%Given a contract $p \in \mathcal{P}$ as input, the \texttt{Action-Oracle} procedure (Algorithm~\ref{alg:action_oracle}) has to decide whether the agent's best response $a^\star(p)$ can be unequivocally associated with some meta-action $d \in \mathcal{D}$ or \emph{not}.
%
%\begin{wrapfigure}[17]{R}{0.55\textwidth}
%\begin{minipage}{0.55\textwidth}
%\begin{algorithm}[H]
%	\caption{\texttt{Action-Oracle}}\label{alg:action_oracle}
%	\begin{algorithmic}[1]
	%		\Require $p \in \mathcal{P}$
	%		\State ${I}_{\omega} \gets 0$ for all $\omega \in \Omega$
	%		\For{$\tau =1 , \ldots, q$}%\Comment{$q$ is set in Algorithm~\ref{alg:learn_contract}}
	%		\State Commit to $p $ and observe $\omega \in \Omega$
	%		\State  ${I}_{\omega} \gets {I}_{\omega}+1$
	%		\EndFor
	%		\State Build $\widetilde{F} \in \Delta_\Omega:  \widetilde F_{\omega} = {I}_{\omega}/q$ for all $\omega \in \Omega$
	%		% \State $ \widetilde F_{\omega} \gets \frac{1}{q} {I}_{\omega}$  for all $\omega \in \Omega$
	%		\If{$\exists ! d \in \mathcal{D} : \exists F \in \mathcal{F}[d] : \| F -   \widetilde F \|_{\infty} \le 2 \epsilon $}\label{eq_action_oracle_condition}
	%		\State $\mathcal{F}[d] \gets \mathcal{F}[d] \cup \{ \widetilde{F} \}$
	%		\State \Return $\big( d, \widetilde F \big)$
	%		\EndIf
	%		\State \Return $\big( \bot, \widetilde F \big)$
	%	\end{algorithmic}
%\end{algorithm}
%\end{minipage}
%\end{wrapfigure}
%
%Algorithm~\ref{alg:action_oracle} works by first prescribing the principal to commit to $p$ for $q \in \mathbb{N}$ consecutive rounds (see Line~\ref{line:set_q} of Algorithm~\ref{alg:final_algorithm} for the definition of $q$).
%%
%This allows to build an an empirical distribution $\widetilde{F} \in \Delta_{\Omega}$ which is an estimate of the (true) distribution over outcomes $F_{a^\star(p)}$ induced by $a^\star(p)$.
%%
%Then, the empirical distribution is compared with those computed during previous runs of Algorithm~\ref{alg:action_oracle}.
%%
%To perform such a comparison, all the empirical distributions computed by the algorithm are stored in a dictionary $\mathcal{F}$ (initialized in Line~\ref{line:set_D_F} of Algorithm~\ref{alg:final_algorithm}), where $\mathcal{F}[d]$ is built so that it contains all the $\widetilde{F} \in \Delta_{\Omega}$ computed by Algorithm~\ref{alg:action_oracle} for contracts $p \in \mathcal{P}$ such that $a^\star(p)$ is associated with the meta-action $d \in \mathcal{D}$.
%
%Based on the outcome of the comparison, Algorithm~\ref{alg:action_oracle} may terminate in two different ways:
%\begin{itemize}
%	\item If there exists a \emph{unique} meta-action $d \in \mathcal{D}$ such that $ \| F -   \widetilde F \|_{\infty} \le 2 \epsilon $ for some $F \in \mathcal{F}[d]$, then the algorithm associates the best-response action $a^\star(p)$ to $d$, and it returns $(d,\widetilde{F})$.
%	%
%	\item In all the other cases, the algorithm cannot unequivocally associate $a^\star(p)$ with one of the meta-actions in $\mathcal{D}$, and, thus, it terminates with the special value $(\bot, \widetilde{F})$ (which will stop the partitioning of $\mathcal{P}$ and result in a call to \texttt{Update-Actions}).
%\end{itemize} 
%
% Intuitively, the procedure described above ensures that $ \|  \widetilde F - F_{a^\star(p)} \|_{\infty} \le \epsilon $ holds with sufficiently high probability.
%
% As a result, if Algorithm~\ref{alg:action_oracle} is run for two different contracts $p, p' \in \mathcal{P}$ such that $a^\star(p) = a^\star(p')$, the resulting empirical distributions are guaranteed to be within $2\epsilon$ of each other with sufficiently high probability, and, thus, they can be associated with the same meta-action.


%For ease of presentation, in the following definition we introduce a \emph{clean event} which allows us to factor out from our analysis the ``with high probability'' statements.
%%
%At the end of the section, we will show that such an event holds with sufficiently high probability.
%%
%\begin{definition}[Clean event]
%	Given any $\epsilon > 0$, we let $\mathcal{E}_\epsilon$ be the event in which Algorithm~\ref{alg:action_oracle} always computes an $\widetilde F \in \Delta_{\Omega}$ such that $ \|\widetilde{F} - F_{a^\star(p)} \|_{\infty} \le \epsilon $, where $p \in \mathcal{P}$ is the input to the algorithm.
%\end{definition}


%The crucial property that Algorithm~\ref{alg:action_oracle} (together with the related \texttt{Update-Actions} procedure described in the following Section~\ref{sec:update_actions}) needs to guarantee is that no action is ever associated with two different meta-actions.
%%
%By letting $\mathcal{P}_d \subseteq \mathcal{P}$ be the set of contracts $p \in \mathcal{P}$ which are given as input to Algorithm~\ref{alg:action_oracle} all the times it computed an empirical distribution $\widetilde F \in \mathcal{F}[d]$, we denote by $I(d) \coloneqq \bigcup_{p \in \mathcal{P}_d} a^\star(p)$ the set of actions associated with the meta-action $d \in \mathcal{D}$.
%%
%Then, the crucial property that needs to be guaranteed is that $I(d) \cap I(d') = \varnothing$ for any two meta-actions $d,d' \in \mathcal{D}$.
%%
%Under the event $\mathcal{E}_\epsilon$, this is clearly maintained by Algorithm~\ref{alg:action_oracle} when it returns a pair $(d,\widetilde{F})$, while in the other case in which the returned pair is $(\bot,\widetilde{F})$ it is a duty of the \texttt{Update-Actions} procedure to guarantee that the property is satisfied, as we show in the following Section~\ref{sec:update_actions}.

%As outlined in Section~\ref{sec:preliminaries}, the principal only observes the realized outcome $\omega \in \Omega$ when committing to a contract, without any knowledge of the agent's actual action. Therefore, we design the \ActionOracle algorithm (see Algorithm~\ref{alg:action_oracle}), which requires the principal to commit $q \in \mathbb{N}$ multiple times to the same contract $p \in \mathcal{P}$ in order to estimate an empirical distribution over outcomes $\widetilde{F} \in \Delta_{\Omega}$. The main idea behind \ActionOracle is to cluster under the same discovered action $d \in \mathcal{D}$ the contracts that result in sufficiently similar empirical distributions. This is beacuse if two contracts implement the same action they will lead to similar empirical distributions with high probability. Before presenting the \ActionOracle algorithm, we introduce the following event which will be useful in the following.
%
%\begin{definition}
%Let $\mathcal{E}_\epsilon$ be the event in which all the calls to \textnormal{\texttt{ACTION-ORACLE}} return an $\tilde F \in \Delta_{\Omega}$ such that $ \|\widetilde{F} - F_{a^\star(p)} \|_{\infty} \le \epsilon $, where $p \in \mathcal{P}$ is the contract given as input to the \textnormal{\texttt{ACTION-ORACLE}} algorithm.
%\end{definition}
%
%As a direct consequence, under the event $\mathcal{E}_\epsilon$, it follows that for any two empirical distributions $\widetilde{F}_1, \widetilde{F}_2 \in \Delta_{\Omega}$ associated with the same agent's action, the following condition holds: $\| \widetilde{F}_1 - \widetilde{F}_2 \|_{\infty} \leq 2\epsilon$. Throughout the execution of Algorithm~\ref{alg:learn_contract}, we maintain a set $\mathcal{F}_d$ that keeps track of all observed empirical distributions associated with the discovered action $d \in \mathcal{D}$. A crucial step occurs when the condition at Line~\ref{eq_action_oracle_condition} in \texttt{ACTION-ORACLE} is not satisfied. In such a case the \texttt{ACTION-ORACLE} algorithms returns the tuple $(\bot, \tilde F)$ being unable to properly classify the contract leading to the empricial distribution  $\widetilde{F}$ in one of the discovered actions $d \in \dreg$. (A better dscussion on how such an alforithm is employed will be gievn in Section~\ref{sec:try_partition}).


%\subsection{\texttt{Update-Actions}}\label{sec:update_actions}


%The \texttt{Update-Actions} procedure (Algorithm~\ref{alg:update_actions}) is called with an empirical distribution $\widetilde{F} \in \Delta_{\Omega}$ as input any time the \texttt{Action-Oracle} procedure returns a pair $(\bot, \widetilde{F})$.


%\begin{wrapfigure}[12]{R}{0.47\textwidth}
%	\begin{minipage}{0.47\textwidth}
	%		\begin{algorithm}[H]
		%			\caption{\texttt{Update-Actions}}\label{alg:update_actions}
		%			\begin{algorithmic}[1]
			%				\Require $\widetilde F \in \widetilde{F}$
			%				\State $\mathcal{D}^\diamond \gets \varnothing$
			%				\For {$d \in \mathcal{D}$}
			%				\If{$\exists F \in \mathcal{F}[d] : \| F -   \widetilde F \|_{\infty} \leq 2 \epsilon$}
			%				\State $\mathcal{D}^\diamond \gets \mathcal{D}^\diamond \cup \{ d \}$
			%				\EndIf
			%				\EndFor
			%				\State $\mathcal{D} \gets \left( \mathcal{D} \setminus \mathcal{D}^\diamond \right) \cup \{ d^\diamond \}$ %\Comment{$d^\diamond$ new meta-action}
			%				\State $\mathcal{F}[{d^\diamond}] \gets \bigcup_{d \in \mathcal{D}^\diamond} \mathcal{F}[d] \cup \{ \widetilde F \}$ 
			%				\State Clear $\mathcal{F}[d]$ for all $d \in \mathcal{D}^\diamond$
			%				% \State \Return $(\mathcal{D}, \{\mathcal{F}_d \}_{d \in \mathcal{D}}) $
			%			\end{algorithmic}
		%		\end{algorithm}
	%	\end{minipage}
%\end{wrapfigure}
%%
%The procedure implemented by Algorithm~\ref{alg:update_actions} jointly deals with two distinct cases:
%\begin{itemize}[leftmargin=6mm]
%	\item If the empirical distribution $\widetilde{F} \in \Delta_{\Omega}$ is such that $\|  {F} - \widetilde{F}\|_{\infty} > 2\epsilon$ for all $d \in \dreg$, $F \in \mathcal{F}[d]$, then $\mathcal{D}^\diamond = \varnothing$ and a brand new meta-action $d^\diamond$ is added to $\mathcal{D}$.
%	%
%	Intuitively, this is done since, under the event $\mathcal{E}_\epsilon$, if $a^\star(p) \in I(d)$ for some $d \in \mathcal{D}$, then it would be the case that $\|{F} - \widetilde{F} \|_{\infty}  \le 2\epsilon$ for some $F \in \mathcal{F}[d]$.
%	%
%	%
%	%
%	\item If instead there exists a subset of meta-actions $\mathcal{D}^\diamond \subseteq \mathcal{D}$ such that there exists $F \in \mathcal{F}[d]$ with $\| F -   \widetilde F \|_{\infty} \leq 2 \epsilon$ for every $d \in \mathcal{D}^\diamond$, then all the meta-actions in $\mathcal{D}^\diamond$ are merged into a single (new) meta-action.
%	%
%	Intuitively, this is done since all the meta-action actions $d \in \mathcal{D}^\diamond$ are such that $a^\star(p) \in I(d)$ under the event $\mathcal{E}_{\epsilon}$.
%\end{itemize}
%
%Notice that, at the end of Algorithm~\ref{alg:update_actions}, the dictionary $\mathcal{F}$ is properly re-organized in order to reflect the new composition of $\mathcal{D}$.
%
%In this case, we rely on the \texttt{UPDATE-ACTIONS} algorithm to update the set of discovered actions $\mathcal{D}$. Specifically, if the observed empirical distribution $\widetilde{F} \in \Delta_{\Omega}$ satisfies the condition $\|\widetilde{F} - {F}\|_{\infty} \geq 2\epsilon$ for every $F \in \mathcal{F}_d$ and $d \in \dreg$, then a new action $d^*$ is discovered. This is because, under the event $\mathcal{E}_\epsilon$, if such an action was already discovered we would have $\|\widetilde{F} - {F} \|_{\infty}  \le 2\epsilon$ for some $F \in \bigcup_{d} \mathcal{F}_d$. Differently from the previous case, if there exists a set of discovered actions $\dreg^* \subseteq \dreg$, such that for each $d \in \dreg^*$ there exists at least one ${F}' \in \mathcal{F}_d$ satisfying $\| {F}' - \widetilde{F} \|_{\infty} \leq 2\epsilon$, then the \texttt{UPDATE-ACTIONS} algorithm merges all the actions in $\dreg^*$ into a single action $d^*$. This is because the distribution $\widetilde{F}$ could potentially be associated to a contract implementing each one of the discovered actions $d \in \mathcal{D}^*$ under the event $\mathcal{E}_{\epsilon}$. Finally, once he \texttt{UPDATE-ACTIONS} algorithm, has updated the new set of discovered actioss associated each observed empirical ditribution observe by the principal to one of the set $\mathcal{F}_d$ it returns the tuple 





%Before discussing some useful properties of the \texttt{UPDATE-ACTIONS} algorithm, we formally introduce a mapping between the set of discovered actions $\dreg$ and the actual set of actions $\mathcal{A}$.
%\begin{definition}
%Let $\mathcal{P}_d \subseteq \mathcal{P}$ be the set of contracts $p \in \mathcal{P}$ given as input to \textnormal{\texttt{ACTION-ORACLE} } all the times it returned an $\tilde F$ such that $\tilde F \in \mathcal{F}_d$. Then we dentote with $I(d) \subseteq \mathcal{A}$ the set such that $I(d) \coloneqq \bigcup_{p \in \mathcal{P}_d} a^\star(p)$.
%\end{definition}
%Intuitively, the set $I(d)\subseteq \mathcal{A}$ is the set containg the action(s) played by the agent that $\textnormal{\texttt{UPDATE-ACTIONS}}$ has identified as a single $d \in \mathcal{D}$ . 

%The following two lemmas show the two key properties of Algorithm~\ref{alg:update_actions}.
%
%\begin{restatable}{lemma}{boundedactions}\label{lem:boundedactions}
%	Under the event $\mathcal{E}_\epsilon$, Algorithm~\ref{alg:update_actions} ensures that, for every meta-action $d \in \mathcal{D}$ and pair of associated actions $a, a' \in I(d)$, it holds $\| F_{a} -   F_{a'} \|_{\infty} \le 5 \epsilon n$.
%	%
%	Moreover, for every $d \in \mathcal{D}$ and empirical distribution $\widetilde{F} \in \mathcal{F}[d]$, it holds $\|\widetilde{F}- F_{a} \|_{\infty} \le 5 \epsilon n $ for all $a \in I(d)$.
%\end{restatable}
%The previous lemma follows from the fact that \ActionOracle aggregate two different actions only if the condition .. is satisfied and by observing that the number of agent's actions is bounded by $n$.

%\begin{restatable}{lemma}{actintersection}\label{lem:nullintersection}
%	Under the event $\mathcal{E}_\epsilon$, Algorithm~\ref{alg:update_actions} ensures that $I(d) \cap I(d') = \varnothing$ for every $d,d' \in \mathcal{D}$.
%\end{restatable}

%\mat{1) vale in alta probabiltà, 2) non ti serve dire che $I(d)\cap I(d')=\emptyset?$} \bac{si vale in alta probabilità ma per quantificarla devi aopere quante volte action oracle viene chiamato}

\end{comment}

